Analyzing Worldwide Social Distancing through Large-Scale Computer Vision

In order to contain the COVID-19 pandemic, countries around the world have introduced social distancing guidelines as public health interventions to reduce the spread of the disease. However, monitoring the efficacy of these guidelines at a large scale (nationwide or worldwide) is difficult. To make matters worse, traditional observational methods such as in-person reporting is dangerous because observers may risk infection. A better solution is to observe activities through network cameras; this approach is scalable and observers can stay in safe locations. This research team has created methods that can discover thousands of network cameras worldwide, retrieve data from the cameras, analyze the data, and report the sizes of crowds as different countries issued and lifted restrictions (also called ''lockdown''). We discover 11,140 network cameras that provide real-time data and we present the results across 15 countries. We collect data from these cameras beginning April 2020 at approximately 0.5TB per week. After analyzing 10,424,459 images from still image cameras and frames extracted periodically from video, the data reveals that the residents in some countries exhibited more activity (judged by numbers of people and vehicles) after the restrictions were lifted. In other countries, the amounts of activities showed no obvious changes during the restrictions and after the restrictions were lifted. The data further reveals whether people stay ''social distancing'', at least 6 feet apart. This study discerns whether social distancing is being followed in several types of locations and geographical locations worldwide and serve as an early indicator whether another wave of infections is likely to occur soon.

==> analysis_failures.tex <==

Some error in computer vision detection is inevitable, and must be accounted for in the analysis of the detection results collected. As explained, the pedestrian detection model had an F1 score of *calculate with new validation set* when sampled with a validation set of 300 images, and hence a fair amount of incorrect and missed detections needs to be expected. The following figures show the error in detections and give insight into the patterns of error. As can be seen in figure A (Jamestown), ... #Add figures here

It is important to note that the resulting plots of detections are heavily influenced by the types of location that the cameras are placed in; some of the locations of the cameras may not be suitable for pedestrian detection and hence misleading in the context of our research. Examples of these cameras in unsuitable locations would be cameras in places that vary in the number of people seasonally such as Ski resort cameras, or cameras that can not capture pedestrians such as rooftop cameras, highway cameras etc. Given the current size of camera data, we cannot perform an analysis on each type of location set of each country. This makes it difficult to make out a definitive conclusion on the effects of social distancing policies of each country as they have a different makeup of camera data that likely do not adequately represent it's nation's activity. Additionally, there is a wide range in the number of cameras collected for each country, which limits the number of countries that can be analyzed.
